The Spectroscopic Data Processing Pipeline for the Dark Energy Spectroscopic Instrument

We describe the spectroscopic data processing pipeline of the Dark Energy Spectroscopic Instrument (DESI), which is conducting a redshift survey of about 40 million galaxies and quasars using a purpose-built instrument on the 4-m Mayall Telescope at Kitt Peak National Observatory. The main goal of DESI is to measure with unprecedented precision the expansion history of the Universe with the Baryon Acoustic Oscillation technique and the growth rate of structure with Redshift Space Distortions. Ten spectrographs with three cameras each disperse the light from 5000 fibers onto 30 CCDs, covering the near UV to near infrared (3600 to 9800 Angstrom) with a spectral resolution ranging from 2000 to 5000. The DESI data pipeline generates wavelength- and flux-calibrated spectra of all the targets, along with spectroscopic classifications and redshift measurements. Fully processed data from each night are typically available to the DESI collaboration the following morning. We give details about the pipeline's algorithms, and provide performance results on the stability of the optics, the quality of the sky background subtraction, and the precision and accuracy of the instrumental calibration. This pipeline has been used to process the DESI Survey Validation data set, and has exceeded the project's requirements for redshift performance, with high efficiency and a purity greater than 99 percent for all target classes.

==> future.tex <==
\section{Future Development Work}
\label{sec:future}

This paper has described the DESI spectroscopic pipeline version used for
the upcoming Early Data Release covering DESI Survey Validation data;
it has additionally been validated on the first year of DESI survey data, to be released in Data Release 1 (DR1).
The algorithms are mature and performing well, thus we do not anticipate major algorithmic changes in the future.  At the same time, we highlight in this section a few areas that may have future development.  If and when significant algorithmic changes are made, those changes will be documented in the corresponding data release papers for the first release including those updates.

Redrock spectral classification and redshift estimation~(\S\ref{sec:redshift})
currently uses
PCA templates to fit the data.  Although this provides speed and flexibility, there is no constraint that the ``best fit'' answer is physically meaningful other than penalizing negative [OII] flux.  This makes Redrock overly sensitive to false fits, especially when there are data problems upstream, e.g.~errors in the background subtraction or flux calibration between the spectrograph arms leading to steps in the spectra.  Future work may introduce archetypes tuned for DESI spectra, non-negative matrix factorization (NMF) templates, or other priors focused on ensuring physically meaningful fits.

The current Redrock galaxy and stellar templates were generated for DESI, but the QSO templates are still the same as those used by BOSS in idlspec2d\cite{Bolton2012}, trained on just a few hundred QSO spectra.  Although there are many more QSO spectra available now that could be used to make improved QSO templates, initial work has found that improving the QSO performance comes at the cost of degrading the completeness of galaxy targets.  Future releases may have new QSO templates tuned to improve QSO performance while preserving the performance of galaxy templates.

The sky subtraction algorithm~(\S\ref{sec:skysubtraction}) is designed for spatially uniform sky, where fiber-to-fiber variations are primarily due to instrumental effects rather than the input sky spectrum actually being different for different fibers.  This is sufficient for dark-time observations and most-bright time observations, though spatial sky gradients during the brightest observations lead to data quality problems.  Explicitely detecting and fitting for non-uniform sky may be included in the future.

The spectral resolution matrix~(\S\ref{sec:extraction}) is not a flux conserving convolution, which may lead to analysis challenges that we have not yet fully understood.  As the DESI collaboration gains experience using these spectra for science analyses, we may learn better ways to model and use the spectral resolution, potentially leading to algorithmic and format updates.

